RobOT: Robustness-Oriented Testing for Deep Learning Systems

Recently, there has been a significant growth of interest in applying software engineering techniques for the quality assurance of deep learning (DL) systems. One popular direction is deep learning testing, where adversarial examples (a.k.a.~bugs) of DL systems are found either by fuzzing or guided search with the help of certain testing metrics. However, recent studies have revealed that the commonly used neuron coverage metrics by existing DL testing approaches are not correlated to model robustness. It is also not an effective measurement on the confidence of the model robustness after testing. In this work, we address this gap by proposing a novel testing framework called Robustness-Oriented Testing (RobOT). A key part of RobOT is a quantitative measurement on 1) the value of each test case in improving model robustness (often via retraining), and 2) the convergence quality of the model robustness improvement. RobOT utilizes the proposed metric to automatically generate test cases valuable for improving model robustness. The proposed metric is also a strong indicator on how well robustness improvement has converged through testing. Experiments on multiple benchmark datasets confirm the effectiveness and efficiency of RobOT in improving DL model robustness, with 67.02% increase on the adversarial robustness that is 50.65% higher than the state-of-the-art work DeepGini.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \cite{year no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> icse21 2/Background.tex <==
\section{Background}
\label{sec:back}

% In this section, we berifly review necessary background to understand this work.

\subsection{Deep Neural Networks}

In this work, we focus on deep learning models, e.g., deep neural networks (DNNs) for classification. 
% We will show later that our approach can be easily adapted to other types of deep learning models. 
% Next, w
We introduce a conceptual deep neural network (DNN) as an example in Fig.~\ref{fig:dnn} for simplicity and remark that our approach is applicable for state-of-the-art DNNs in our experiments like ResNet \cite{resnet}, VGG \cite{vgg}, etc.

\paragraph*{DNN}
\label{subsec:DNN}
A DNN classifier is a function $f:X\to Y$, which maps an input $x\in X$ (often preprocessed into a vector) into a label in $y\in Y$. As shown in Fig.~\ref{fig:dnn}, a DNN $f$ often contains an input layer, multiple hidden layers and an output layer. We use $\theta$ to denote the parameters of $f$ which assigns weights to each connected edge between neurons. 
% We denote these layers as $L = \{ L_{j}|j \in \{0, \dots, n \} \}$ and assume the $j$-th layer has $s_j$ neurons. 
Given an input $x$, we can obtain the output of each neuron on $x$, i.e., $f(x,ne)$, by calculating the weighted sum of the outputs of all the neurons in its previous layer and then applying an activation function (e.g., Sigmoid, hyperbolic tangent (tanh), or rectified linear unit (relu)) $\phi$. Given a dataset $D=\{(x_i,y_i)\}_{i=1}^n$, a DNN is often trained by solving the following optimization problem:
\begin{equation}
\min_\theta\frac{1}{n}\sum_{i=1}^n \mathcal{J}(f_\theta(x_i),y_i)
\end{equation}
, where $\mathcal{J}$ is a loss function which calculates a loss by comparing the model output $f_\theta(x_i)$ with the ground-truth label $y_i$. The most commonly used loss function for multi-class classification tasks is the categorical cross-entropy. The DNN is then trained by computing the gradient w.r.t. the loss for each sample in $D$ and updating $\theta$ accordingly.
% \begin{equation}
% \label{equation:neuron}
% v_{j,k} = \phi(\sum_{l=1}^{s_{j-1}} \omega_{j-1,k,l} \cdot v_{j-1, l})
% \end{equation}
% In the following, we use $\theta = \{\omega_{j,k} | 1 \leq j \leq J, 0 \leq k \leq s_j\}$ to denote the set of parameters of $f$. 
% A DNN with $n$ layers can thus be viewed as the concatenation of layers $f=f_1\circ f_2\cdots f_n$. 
% % In this work, we focus on DNN classifiers $\mathcal{D}: X \to Y$, i.e., for a given instance $x \in X$, a DNN outputs a predicted label $y \in Y$ which has the highest probability.

\begin{figure}[t]
\centering
% \includesvg{framework}
\includegraphics[width=0.35\textwidth]{dnn.pdf}
\caption{An example DNN to predict cat or dog.}
\label{fig:dnn}
\end{figure}

\subsection{Deep Learning Testing} Most existing deep learning testing works are based on neuron coverage \cite{deepxplore} or its variants \cite{deepgauge}. Simply speaking, a neuron $ne$ is covered if there exists at least one test case $x$ where $f(x,ne)$ is larger than a threshold and thus been activated. We omit the details of other variants and briefly introduce the following testing methods as representatives. We also provide pointers for more details.

\vspace{1mm}
\noindent\textbf{DeepXplore} \cite{deepxplore} is the first testing work for DNN. DeepXplore proposed the first testing metric, i.e., neuron coverage and a differential testing framework to generate test cases to improve the neuron coverage.

\vspace{1mm}
% \noindent\textbf{Concolic Testing} \cite{concolic}\\
\noindent\textbf{DeepHunter} \cite{deephunter} is a fuzzing framework which randomly selects seeds to fuzz guided by multi-granularity neuron coverage metrics defined in \cite{deepgauge}.

\vspace{1mm}
\noindent\textbf{ADAPT} \cite{adapt} is another recent work which adopts multiple adaptive strategies to generate test cases which could improve the multi-granularity neuron coverage metrics defined in \cite{deepgauge}.

\vspace{1mm}
\noindent\textbf{Adversarial Attacks} Beside the above testing methods, traditional adversarial attacks like FGSM \cite{fgsm}, JSMA \cite{jsma}, C\&W \cite{cw} and PGD \cite{pgd} attacks are also used to generate test cases in multiple works. 


\subsection{Problem definition} 
% Assume a testing pipeline as shown in Fig.~\ref{}.\jy{formalized in Sec.~\ref{sec:qat}} 
Unlike existing coverage guided testing works, our goal is to design a robustness-oriented testing framework to improve the DL model robustness by testing. Two key problems are to be answered: 1) how can we design testing metrics which are strongly correlated with model robustness? 2) how can we automatically generate test cases favoring the proposed testing metrics?

==> icse21 2/Conclusion.tex <==
\section{Conclusion}
\label{sec:con}

In this work, we propose a novel robustness-oriented testing framework RobOT for deep learning systems towards improving model robustness against adversarial examples. The core of RobOT is a metric called FOL to quantify both the value of each test case in improving model robustness (often via retraining) and the convergence quality of the model robustness improvement. We also propose to utilize the proposed metric to automatically fuzz for more valuable test cases to improve model robustness. 
% Meanwhile FOL is also a strong indicator of how well the robustness improvement has converged by testing. 
We implemented RobOT as a self-contained open-source toolkit. Our experiments on multiple benchmark datasets verify the effectiveness and efficiency of RobOT in improving DL model robustness, i.e., with 67.02\% increasement on the adversarial robustness that is 50.65\% higher than the state-of-the-art work DeepGini.

==> icse21 2/Experiment.tex <==
\section{Experimental Evaluation}
\label{sec:exp}

We have implemented RobOT as a self-contained tookit with about 4k lines of Python code. The source code and all the experiment details are available at \cite{code}. In the following, we evaluate RobOT through multiple experiments.

\subsection{Experiment Settings}

\paragraph{Datasets and Models} We adopt four widely used image classification benchmark datasets for the evaluation. We summarize the details of the datasets and models used in Tab. \ref{tb:ds}. 
% For each dataset, we train two models of different complexity with details shown in Tab.~\ref{tb:md}.


% \begin{table}[t]
% \centering
% \caption{Models.}
% \begin{tabular}{|l|llll|}
% \hline
% Dataset       & Model 1 & Accuracy & Model 2 & Accuracy \\ \hline
% MNIST         &         &          &         &          \\
% SVHN          &         &          &         &          \\
% Fashion-MNIST &         &          &         &          \\
% CIFAR10       &         &          &         &          \\
% \hline
% \end{tabular}
% \label{tb:md}
% \end{table}

\paragraph{Test Case Generation} We adopt two kinds of adversarial attacks and three kinds of coverage-guided testing approaches
to generate test cases for the evaluation in the following. 



% \begin{itemize}
%    \item FGSM \cite{fgsm} is a gradient-guided one-step adversarial attack. The required parameter is to control the scale of the perturbation.
%    \item PGD \cite{pgd} is a gradient-guided multi-step adversarial attack. The required parameters are the maximum perturbation and a step size.
%    \item DeepXplore \cite{deepxplore} is the first testing framework which is designed to improve neuron coverage metric. The required parameters are...
%    \item DLFuzz \cite{dlfuzz} is a DL fuzzing framework to maximize neuron coverage and the prediction difference. The required parameters are... 
%    \item ADAPT \cite{adapt} is the state-of-the-art test case generation algorithm to improve multi-granularity neuron coverage metrics. The required parameters are...
% \end{itemize}
We summarize all the configurations of the test case generation algorithms in Tab.~\ref{tb:tg}.


\paragraph{Test Case Selection Baseline} We adopt the most recent work DeepGini \cite{deepgini} as the baseline of the test case selection strategy. DeepGini calculates a Gini index for each test case according to the output probability distribution of the model. A test case with larger Gini index is considered more valuable for improving model robustness.

\paragraph{Robustness Evaluation} We adopt Def. \ref{def:empirical-robustness} to empirically evaluate a model's robustness. In practice, we compose a validation set of adversarial examples $D_v$ for each dataset by combining the adversarial examples generated using both FGSM and PGD (10000 each). The attack parameters are the same with Tab. \ref{tb:tg}. We then evaluate a model's robustness by calculating its accuracy on $D_v$. 


\begin{table}[]
\centering
\caption{Datasets and models.}
\begin{tabular}{|l|llll|}
\hline
Dataset       & Training & Testing & Model     & Accuracy \\ \hline
MNIST         & 60000    & 10000   & LeNet-5   & 99.02\%  \\
Fashion-MNIST & 60000    & 10000   & LeNet-5   & 90.70\%  \\
SVHN          & 73257    & 26032   & LeNet-5   & 88.84\%  \\
CIFAR10       & 50000    & 10000   & ResNet-20 & 90.39\%  \\
\hline
\end{tabular}
\label{tb:ds}
\end{table}


\begin{table}[]
\centering
\caption{Test case generation details.}
\scalebox{0.74}{
   \begin{tabular}{|l|l|llll|}
\hline
Testing Method & Parameter      & MNIST & SVHN   & Fashion-MNIST & CIFAR10 \\ \hline
FGSM           & Step size      & 0.3   & 0.03   & 0.03          & 0.01    \\
               % & \# Test case    &       &        &               &         \\ \hline
PGD            & Steps          & 10    & 10     & 10            & 10      \\
               & Step size      & 0.3/6 & 0.03/6 & 0.3/6        & 0.01/6  \\
               % & \# Test case    &       &        &               &         \\ \hline
DeepXplore     & Relu threshold & 0.5   & 0.5    & 0.5           & 0.5     \\
               % & \# Test case    &       &        &               &         \\ \hline
DLFuzz/ADAPT   & Time per seed  & 10 s    & 10 s     & 10 s            & 20 s      \\
               & Relu threshold & 0.5   & 0.5    & 0.5           & 0.5     \\
% DLFuzz         & \# Test case    &       &        &               &         \\ \hline

\hline
\end{tabular}
}

\label{tb:tg}
\end{table}

\subsection{Research Questions}
% We aim to answer the following research questions through our experiments.

\vspace{1mm}
\noindent\textbf{RQ1: What is the correlation between our FOL metric and model robustness?} To answer this question, we first select three models with different robustness levels for each dataset. The first model (Model 1) is the original trained model. The second model (Model 2) is a robustness-enhanced model which is retrained\footnote{Retaining in this work takes 10 (40 for CIFAR10) additional epochs based on the original model.} by augmenting 5\% of the generated test cases and is more robust than Model 1. The third model (Model 3) is a robustness-enhanced model which is retrained by augmenting 10\% of the generated test cases and is most robust. Then, for each model, we conduct adversarial attacks to obtain a same number (10000 for FGSM and 10000 for PGD) of adversarial examples. 


\begin{figure*}[t]
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/mnist_fol_distribution.pdf}
   % \caption{NASA Logo} 
   \label{fig:fol:mnist}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/fashion_fol_distribution.pdf}
   % \caption{Orion Logo} 
   \label{fig:fol:fashion}
\end{subfigure}%
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/svhn_fol_distribution.pdf}
   % \caption{NASA Logo} 
   \label{fig:fol:svhn}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/cifar_fol_distribution.pdf}
   % \caption{Orion Logo} 
   \label{fig:fol:cifar}
\end{subfigure}%
   \caption{FOL distribution of adversarial examples for models with different robustness.}
   \label{fig:fol}
\end{figure*}

We show the FOL distribution of the adversarial examples for different models in Fig. \ref{fig:fol}. We observe that there is a strong correlation between the FOL distribution of adversarial examples and the model robustness. Specifically, \emph{the adversarial examples of a more robust model have smaller FOL values.} This is clearly evidenced by Fig. \ref{fig:fol}, i.e., for every dataset, the probability density is intensively distributed around zero for Model 3 (the most robust model) while is steadily expanding to larger FOL values for Model 2 and Model 1 (with Model 1 larger than Model 2). The underlying reason is that a more robust model in general has a more \emph{flat} loss distribution and thus a smaller FOL value (since it is based on the loss gradient). 

\begin{figure}[t]
\centering 
\includegraphics[width=.33\textwidth]{figs/fgsm-pgd_fol_distribution.pdf}
\caption{FOL distribution of adversarial examples from FGSM and PGD for CIFAR10 model.} 
\label{fig:fol:com}
\end{figure}

In addition, we also observe that adversarial examples crafted by stronger attacks have smaller FOL values. Fig. \ref{fig:fol:com} shows the FOL distribution of adversarial examples from attacking the CIFAR10 model with FGSM and PGD respectively. We could observe that adversarial examples from PGD have significantly smaller FOL values than FGSM. The reason is that stronger attacks like PGD are generating adversarial examples that have better loss convergence quality and induce higher loss. 

We thus have the following answer to RQ1:
\begin{framed}
\noindent \emph{Answer to RQ1: FOL is strongly correlated with model robustness. A more robust model have smaller FOL values for adversarial examples.
}\end{framed}       

% In addition, we have the following observations.
% \begin{itemize}
%    \item Adversarial examples from stronger attacks have smaller FOL values. Fig. \ref{} shows the FOL distribution of adversarial examples from attacking CIFAR10 model with FGSM and PGD attack respectively. We could observe that adversarial examples from PGD attack has smaller FOL values than FGSM attack. The reason is that stronger attacks often have better loss convergence quality and induce higher loss.
%    % \item There are two cases when FOL will be zero.
% \end{itemize}




% Possible experiments:
% \begin{itemize}
% 	\item Select a set of test image, run FGSM and PGD respectively with different $\epsilon-$bounds, compare the FOSC of the resulting adversarial samples. \jy{The goal is to show that PGD can generate test cases with higher quality than FGSM, which is intuitive but FOSC provides a quantitative way to measure such a goodness.}
% 	\item For PGD alone, show the change of FOSC values during the PGD iteration. \jy{it is interesting to see it drops to 0 when a large bound is given, which might be useful for selecting the approriate bound for testing.}
% \end{itemize}


% Intuition: the worst case in the loss landscape will improve the model most.
% \begin{remark}This part is mostly done, we just need to wrap things up.\end{remark}





\vspace{1mm}
\noindent\textbf{RQ2: How effective is our FOL metric for test case selection?} To answer the question, we first generate a large set of test cases using different methods, and then adopt different test case selection strategies (i.e., BE-ST, KM-ST and DeepGini) to select a subset of test cases with the same size to retrain the model. A selection strategy is considered more effective if the retrained model with the selected test cases is more robust.

We distinguish two different kinds of test case generation algorithms which are both used in the literature, i.e., adversarial attacks and neuron coverage-guided algorithms, for more fine-grained analysis. For adversarial attacks, we adopt FGSM (weak) and PGD (strong) attacks to generate a combined set of test cases. For DeepXplore, DLFuzz and ADAPT, we generate a set of test cases for each of them. The parameters used are consistent with Tab. \ref{tb:tg}. For each set of test cases, we use BE-ST, KM-ST and DeepGini strategy respectively to select x (ranging from 1 to 10) percent of them to obtain a retrained model and evaluate its model robustness. 


\begin{figure*}[t]
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/mnist_attack_robustness.pdf}
   % \caption{NASA Logo} 
   \label{fig:ts:mnist}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/fashion_attack_robustness.pdf}
   % \caption{Orion Logo} 
   \label{fig:ts:fashion}
\end{subfigure}%
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/svhn_attack_robustness.pdf}
   % \caption{NASA Logo} 
   \label{fig:ts:svhn}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/cifar_attack_robustness.pdf}
   % \caption{Orion Logo} 
   \label{fig:ts:cifar}
\end{subfigure}%

\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/mnist_xplore_robustness.pdf}
   % \caption{NASA Logo} 
   \label{fig:ts:mnist}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/fashion_xplore_robustness.pdf}
   % \caption{Orion Logo} 
   \label{fig:ts:fashion}
\end{subfigure}%
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/svhn_xplore_robustness.pdf}
   % \caption{NASA Logo} 
   \label{fig:ts:svhn}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/cifar_xplore_robustness.pdf}
   % \caption{Orion Logo} 
   \label{fig:ts:cifar}
\end{subfigure}%

\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/mnist_dlfuzz_robustness.pdf}
   % \caption{NASA Logo} 
   \label{fig:ts:mnist}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/fashion_dlfuzz_robustness.pdf}
   % \caption{Orion Logo} 
   \label{fig:ts:fashion}
\end{subfigure}%
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/svhn_dlfuzz_robustness.pdf}
   % \caption{NASA Logo} 
   \label{fig:ts:svhn}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/cifar_dlfuzz_robustness.pdf}
   % \caption{Orion Logo} 
   \label{fig:ts:cifar}
\end{subfigure}%

\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/mnist_adapt_robustness.pdf}
   % \caption{NASA Logo} 
   \label{fig:ts:mnist}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/fashion_adapt_robustness.pdf}
   % \caption{Orion Logo} 
   \label{fig:ts:fashion}
\end{subfigure}%
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/svhn_adapt_robustness.pdf}
   % \caption{NASA Logo} 
   \label{fig:ts:svhn}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/cifar_adapt_robustness.pdf}
   % \caption{Orion Logo} 
   \label{fig:ts:cifar}
\end{subfigure}%

   \caption{Test case selection and robustness improvement with different strategies.}
   \label{fig:ts}
\end{figure*}

Fig. \ref{fig:ts} shows the results. We observe that for all the strategies, the retrained model obtained improved resilience to adversarial examples to some extent. Besides, the model's robustness steadily improves as we augment more test cases (from 1\% to 10\%) for retraining. However, we could also observe that in almost all cases (except 1 case), our FOL guided strategies (both BE-ST and KM-ST) have significantly better performance than DeepGini, i.e., achieving 30.48\%, 84.62\%, 54.91\% and 35.92\% more robustness improvement on average for the four different sets of test cases. The reason is that FOL is able to select test cases which have higher and more diverse loss than DeepGini (as shown in Fig. \ref{fig:loss:st} previously), which are better correlated with model robustness. Meanwhile, we observe that the retrained models maintain high accuracy on the test set as well (as summarized in Tab. \ref{tb:acc}).  

Besides, we observe that different test case generation algorithms obtain different robustness improvements. Among DeepXplore, DLFuzz and ADAPT, ADAPT and DLFuzz have the highest (53.39\% on average) and lowest (31.18\% on average) robustness improvement respectively while DeepXplore is in the middle (48.36\% on average). Adversarial attacks often achieve higher robustness improvement than all three neuron coverage-guided fuzzing algorithms for simpler datasets such as MNIST, Fashion-MNIST and SVHN. This casts shadow on the usefulness of the test cases generated by neuron coverage-guided fuzzing algorithms in improving model robustness and is consistent with \cite{limit,misleading,meaningless}. 

% \jy{attack is the best...}
% We further conduct experiments to evaluate how robust the retrained models with adversarial examples from adversarial attacks are against adversarial examples from different testing algorithms. 
We further conduct experiments to evaluate and compare how robust the retrained models are when using adversarial examples generated in different ways: one from the attacks (Fig. \ref{fig:ts}), and the other from different testing algorithms. 
We summarize the result in Tab. \ref{tb:trans}. We observe that the robustness drops noticeably (which is especially the case for CIFAR10), i.e., 18.64\%, 26.41\% and 23.09\% for DeepXplore, DLFuzz, and ADAPT each on average (compared to the results in Fig. \ref{fig:ts}). Nevertheless, our test case selection strategies still outperform DeepGini in all cases. This shows that adversarial examples from adversarial attacks alone are insufficient. It is necessary to improve the diversity of test cases for retraining from a perspective that is well correlated with model robustness.   


% Cross-validation, does retrain with attack inputs generalize to test cases?


\begin{table}[]
\centering
\caption{Test accuracy of model before and after retraining with 10 percent of generated test cases using adversarial attacks.}
\begin{tabular}{|l|ll|}
\hline
Dataset       & Original & Retrained \\ \hline
MNIST         & 99.02\%  & 98.95\%   \\
Fashion-MNIST & 90.70\%  & 90.63\%   \\
SVHN          & 88.84\%  & 87.13\%   \\
CIFAR10       & 90.39\%  & 90.13\%   \\
\hline
\end{tabular}
\label{tb:acc}
\end{table}

\begin{table*}[]
\caption{Robustness performance of models (retrained using adversarial examples from attack algorithms)
against test cases generated by DL testing tools.}
\centering
\scalebox{0.85}{
\begin{tabular}{|l|llll|llll|llll|}
\hline
              & DeepXplore &         &          &         & DLFuzz  &         &          &         & ADAPT   &         &          &         \\ \cline{2-13}
Dataset       & BE-ST      & KM-ST   & DeepGini & Average     & BE-ST   & KM-ST   & DeepGini & Average     & BE-ST   & KM-ST   & DeepGini & Average     \\ \hline
MNIST         & 86.12\%    & 80.56\% & 73.74\%  & \textbf{80.14\%} & 76.39\% & 74.73\% & 65.59\%  & \textbf{72.24\%} & 82.60\% & 75.68\% & 70.36\%  & \textbf{76.21\%} \\
Fashion-MNIST & 51.57\%    & 47.97\% & 34.14\%  & \textbf{44.56\%} & 38.15\% & 35.44\% & 27.16\%  & \textbf{33.58\%} & 50.55\% & 47.50\% & 31.92\%  & \textbf{43.32\%} \\
SVHN          & 37.10\%    & 38.29\% & 27.26\%  & \textbf{34.55\%} & 32.83\% & 34.83\% & 25.34\%  & \textbf{31.00\%} & 25.71\% & 28.51\% & 19.15\%  & \textbf{24.46\%} \\
CIFAR10       & 25.25\%    & 20.16\% & 12.92\%  & \textbf{19.44\%} & 18.28\% & 14.20\% & 9.31\%   & \textbf{13.93\%} & 22.37\% & 18.48\% & 12.08\%  & \textbf{17.64\%} \\ \hline

Average       & \textbf{50.01\%}    & \textbf{46.75\%} & \textbf{37.01\%}  &  & \textbf{41.41\%} & \textbf{39.8\%} & \textbf{31.85\%}   &  & \textbf{45.31\%} & \textbf{42.54\%} & \textbf{33.36\%}  &  \\
\hline
\end{tabular}
}
\label{tb:trans}
\end{table*}

\begin{table*}[]
\centering

\caption{Comparison of FOL-fuzz and ADAPT. $a/b$: a is the result of FOL-fuzz and b is the result of ADAPT.}

\begin{tabular}{|l|ll|ll|ll|}
\hline
              & 5 min       &            & 10 min      &            & 20 min      &            \\ \cline{2-7}
Dataset       & \# Test case & Robustness$\uparrow$ & \# Test case & Robustness$\uparrow$ & \# Test case & Robustness$\uparrow$ \\ \hline
MNIST         & 1692/2125        & 33.62\%/18.73\%       & 3472/4521        & 48.04\%/36.46\%       & 7226/8943        & 68.02\%/54.38\%       \\
Fashion-MNIST & 4294/5485        & 40.75\%/6.74\%        & 8906/10433       & 53.88\%/14.94\%       & 18527/21872       & 69.03\%/27.24\%       \\
SVHN          & 6236/8401        & 24.25\%/21.3\%       & 12465/17429       & 30.42\%/27.52\%       & 24864/33692       & 39.99\%/34.51\%    \\
CIFAR10       &      1029/1911     &     18.62\%/17.03\%       &   2006/3722          &     22.07\%/18.12\%       &       4050/6947      &     27.36\%/20.54\%       \\
\hline
Average       &      \textbf{3313/4480}    &  \textbf{29.31\%/15.95\%}          &    \textbf{6712/9026}         &    \textbf{38.6\%/24.26\%}        &       \textbf{13667/17864}      &  \textbf{51.1\%/34.17\%}          \\
\hline
\end{tabular}

\label{tb:fuzz}
\end{table*}

We thus have the following answer to RQ2:
\begin{framed}
\noindent \emph{Answer to RQ2: FOL guided test case selection is able to select more valuable test cases to improve the model robustness by retraining.
}\end{framed}



% The goal is to show FOSC value can be used for test selection from large set of test cases to reduce retraining cost.
% Possible experiments:
% \begin{itemize}
% 	\item Form a retraining set using different test selection technique, like ISSTA 20 Gini index, uncertainty, or ISSTA 20 Adaptive (prefer small distance), retrain the original model to show the robustness improvement against different attacks or in terms of robustness metrics like CLEVER. Maybe vary the size of the retaining set to show that we don't need a lot of test cases to improve the model.
% \end{itemize}


% \vspace{1mm}
% \noindent\textbf{RQ3: How effective are different testing methods in the perspective of our FOL metric?}\\
% The goal is to show that most existing coverage-oriented testing methods neglects the loss perspective.
% Possible experiments:
% \begin{itemize}
% 	\item Select a set of test image, run different testing methods with a certain $\epsilon-$bound, compare the FOSC value (in terms of certain statistics like mean, variance, etc) of the resulting test cases.
% 	\item Show the correlation between the coverage and the FOSC value. For instance, from a same large test suites using a testing method, form two test suits which aim to improve coverage metrics and FOSC respectively. A possible way to form the test suites is as follows. Select a set of 10000 seeds from test set, for each seed, select top-$k$ test cases in terms of improving coverage and FOSC respectively.
% \end{itemize}

% \begin{remark}Testing methods: ISSTA 20 adaptive, ISSTA 19 coverage-guided fuzzing, ICSE 18 transformation, SOSP 17 deepxplore. Not sure if Youcheng's work can fit in for large networks, need @Youcheng's advice.\end{remark}



\vspace{1mm}
\noindent\textbf{RQ3: How effective and efficient is our FOL guided fuzzing algorithm?} To answer the question, we compare our FOL guided fuzzing algorithm (FOL-Fuzz) with state-of-the-art neuron coverage-guided fuzzing algorithm ADAPT as follows. We run FOL-fuzz and ADAPT for a same period of time, (i.e., 5 minutes, 10 minutes and 20 minutes) to generate test cases. Then we retrain the model with the test cases to compare their robustness improvement. 
% Second, we use FOL-fuzz and ADAPT to generate a same number of xx test cases to compare the time needed. We retrain the model to compare the robustness improvement as well. 
The hyper-parameters for FOL-Fuzz are set as follows: $\xi=10^{-18},\ k=5,\ \lambda=1,\ iters=3,\ learning\_rate=0.1$. The parameters for ADAPT are consistent with Tab. \ref{tb:tg}.    



Tab. \ref{tb:fuzz} shows the results. We could observe that within the same time limit, ADAPT generates slightly more adversarial examples, i.e., 10457 compared to 7897 of FOL-Fuzz. A closer look reveals that ADAPT tends to generate a lot of test cases around a seed towards improving the neuron coverage metrics. However, not all these tests are meaningful to improve model robustness. On the other hand, FOL-Fuzz is able to discover more valuable test cases. We could observe that using FOL-Fuzzed test cases (although less than ADAPT) to retrain the model significantly improves the model's robustness than ADAPT, i.e., 39.67\% compared to 24.79\% of ADAPT on average. 
% Besides, given a same number of seeds, FOL-fuzz is able to generate more valuable test cases for retraining, i.e., achieving xx\% more robustness improvement, in much less time, i.e., xx compared to xx.

We thus have the following answer to RQ3:
\begin{framed}
\noindent \emph{Answer to RQ3: FOL-Fuzz is able to efficiently generate more valuable test cases to improve the model robustness.
}\end{framed}

\subsection{Threats to Validity}

First, our experiments are based on a limited set of test subjects in terms of datasets, types of adversarial attacks and neuron coverage-guided test case generation algorithms. Although we included strong adversarial attack like PGD and state-of-the-art coverage-guided generation algorithm ADAPT, it might be interesting to investigate other attacks like C\&W \cite{cw} and JSMA \cite{jsma}, and fuzzing algorithms like DeepHunter \cite{deephunter}. Second, we adopt an empirical approach to evaluate the model robustness which might be different with different kinds of attacks used. So far it is still an open problem as for how to efficiently measure the robustness of DL models. We do not use more rigorous robustness metric like CLEVER \cite{clever} because it is input-specific and has high cost to calculate (e.g., hours for one input).
Third, our testing framework requires a robustness requirement as input which could be application-specific and is relevant to the model as well. In practice, users could 
% make trials and run testing for iterations and 
adjust the requirement dynamically. 

% the detection algorithm will have some false positives. Since our detection algorithm is threshold-based, there will be some false alarms along with the detection. Meanwhile, there is a tradeoff between avoiding false positives or false negatives as discussed above (i.e., in the selection of $\rho$). Thirdly, the detection of normal samples typically needs more mutations. The reason is that we choose to test against $\varsigma_{nor}$ since we do not know $\varsigma_{adv}$ for an unknown attack. Since normal samples have lower LCR under mutated models in general, they would need more mutations than adversarial samples to draw a conclusion.

% \vspace{1mm}
% \noindent\textbf{RQ4: What is the cost of calculating FOSC metric?}\\

% Compare the cost of calculating coverage metrics and FOSC. FOSC is much more lightweight without any profiling. Take a same set of images, compare the average time of calculating FOSC and the various coverage metrics.


% \textit{Random thoughts:} I totally agree with Xingjun in that our experiments should focus on the standard pipeline of testing. So let's leave the training tricks like dynamic iterative training to future work and simply use naive retraining in this work.

==> icse21 2/Introduction.tex <==
\section{Introduction}

Deep learning (DL) \cite{dl} has been the core driving force behind the unprecedented breakthroughs in solving many challenging real-world problems such as object recognition \cite{cv} and natural language processing \cite{nlp}.
Despite the success, deep learning systems are known to be vulnerable to adversarial examples (or attacks), which are slightly perturbed inputs that are imperceptibly different from normal inputs to human observers but can easily fool state-of-the-art DL systems into making incorrect decisions \cite{fgsm,cw,ma2018characterizing,jiang2019black,wu2020skip}. 
% In the case of images, the perturbations required to subvert the prediction of a well-trained DL model is imperceptible even to human observers.
% subject to adversarial attacks which are able to comprise the decisions of a well-trained deep learning model only by introducing a human-imperceptible subtle change on the original input (a.k.a. adversarial examples) . 
This not only compromises the reliability and robustness of DL systems, but also raises security concerns on their deployment in safety-critical applications such as face recognition \cite{face}, malware detection \cite{md}, medical diagnosis \cite{finlayson2019adversarial,ma2020understanding} and autonomous driving \cite{av,duan2020adversarial}.
% This throws shadow on applying deep learning in safety-critical systems like autonomous driving \cite{av}, malware detection \cite{md} and face recognition \cite{face}, where tremendous loss or even human life might be at risk.

Noticeable efforts have been made in the software engineering community to mitigate the threats of adversarial examples and to improve the robustness of DL systems in the presence of adversarial examples \cite{deeppoly,deepxplore,wang2019adversarial}. Among them, formal verification aims to prove that no adversarial examples exist in the neighborhood of a given input. Substantial progress has been made using approaches like abstract interpretation \cite{deeppoly,yang2020improving} and reachability analysis \cite{star}. However, formal verification techniques are in general expensive and only scale to limited model structures and properties (e.g., local robustness \cite{huang2017safety}). 

Another popular line of work is deep learning testing, which aims to generate test cases that can expose the vulnerabilities of DL models. The test cases can then be used to improve the model robustness by retraining the model, \emph{however, this should not be taken as granted}, as recent studies have shown that test cases generated based on existing testing metrics have limited correlation to model robustness and robustness improvement after retraining~\cite{limit,meaningless}. In this work, we highlight and tackle the problem of effectively generating test cases for improving the adversarial robustness of DL models. 

\begin{figure*}[t]
\centering
\includegraphics[width=0.65\textwidth]{framework.pdf}
\caption{Overview of RobOT testing framework.}
\label{fig:frame}
\end{figure*}

% \todo{DX: not clear why} 


% \todo{DX: better consistent, either DL system or model}
There are two key elements when it comes to testing DL systems. The first element is the testing metric used to evaluate the quality of a test case or a test suite. Multiple testing metrics, including neuron coverage~\cite{deepxplore}, multi-granularity neuron coverage~\cite{deepgauge} and surprise adequacy~\cite{surprise}, have been proposed. The common idea is to explore as much diversity as possible of a certain subspace defined based on different abstraction levels, e.g., neuron activation~\cite{deepxplore}, neuron activation pattern~\cite{deepgauge}, neuron activation conditions~\cite{concolic}, and neuron activation vector~\cite{surprise}. The second key element is the method adopted for test case generation, which is often done by manipulating a given seed input with the guidance of the testing metric. Existing test case generation techniques such as DeepXplore~\cite{deepxplore}, DeepConcolic~\cite{concolic}, DeepHunter~\cite{deephunter} and ADAPT~\cite{adapt} are mostly designed to improve the neuron coverage metrics of the test cases.
% \todo{DX: not clear relating to test case generation}
While existing testing approaches are helpful in exposing vulnerabilities of DL systems to some extent, recent studies have found that neuron coverage metrics are not useful for improving model robustness~\cite{limit,misleading,meaningless}. As a consequence, unlike in the case of traditional program testing (where the program is surely improved after fixing bugs revealed through testing), one may not improve the robustness of the DL system after testing.
 % (e.g., robustness) after generating a set of test cases and retraining the model.  


In this work, we address the above-mentioned limitations of existing DL testing approaches by proposing a novel DL testing framework called RobOT (i.e., \textit{Rob}ustness-\textit{O}riented \textit{T}esting), which integrates the DL (re)training with the testing. 
As illustrated in Fig.~\ref{fig:frame}, RobOT distinguishes itself from existing neuron coverage guided testing works in the following important aspects. First, RobOT is robustness-oriented. RobOT takes a user-defined requirement on the model robustness as input and integrates the retraining process into the testing pipeline. RobOT iteratively improves the model robustness by generating test cases based on a testing metric and retraining the model. Second, in RobOT, we propose a novel set of lightweight metrics that are strongly correlated with model robustness. The metrics can quantitatively measure the relevance of each test case for model retraining, and are designed to favor test cases that can significantly improve model robustness, which is in contrast to existing coverage metrics that have little correlation with model robustness. Furthermore, the proposed metrics can in turn provide strong evidence on the model robustness after testing. 
% \todo{DX: more clear} 
The output of RobOT is an enhanced model that satisfies the robustness requirement.

In a nutshell, we make the following contributions.

\begin{itemize}
\item We propose a robustness-oriented testing (RobOT) framework for DL systems. 
% \todo{DX: We propose a robustness-oriented testing...which is novel for deep learning testing field.}
RobOT provides an end-to-end solution for improving the robustness of DL systems against adversarial examples.

\item We propose a new set of lightweight testing metrics that quantify the importance of each test case with respect to the model's robustness, which are shown to be stronger indicators of the model's robustness than existing metrics.

\item We implement in RobOT, a set of fuzzing strategies guided by the proposed metrics to automatically generate high-quality test cases for improving the model robustness.

\end{itemize}

RobOT is publicly available as an open-source self-contained toolkit \cite{code}.
Experiments on four benchmark datasets confirm the effectiveness of RobOT in improving model robustness. Specifically, RobOT achieves 50.65\% more robustness improvement on average compared to state-of-the-art work DeepGini~\cite{deepgini}.

% The remainder of the paper is organized as follows. We provide background in Sec.~\ref{sec:back}. We then present our detailed approach in Sec.~\ref{sec:meth} and the experiment results in Sec.~\ref{sec:exp}. We discuss related works in Sec.~\ref{sec:rel} and conclude in Sec.~\ref{sec:con}.

==> icse21 2/Methodology.tex <==
\section{The RobOT Framework}
\label{sec:meth}
% Quality assurance-> Proposed framework: utility requirement: robustness/accuracy-> testing-> adversarial samples-> model improvement mechanism: adversarial training/retraining->new model?-> \textit{convergence}

% Contribution: make testing clear, how should we test machine learning models properly.

In this section, we present RobOT, a novel robustness-oriented framework for testing and re-training DL systems.
% future directions: evaluate mechanisms?
The overall framework of RobOT is shown in Figure~\ref{fig:frame}. We assume that \emph{a requirement on the model robustness} (Section \ref{sec:robustness}) is provided in prior for quality assurance
 % (in terms of a certain modle utility of concern) 
purpose. Note that the requirement is likely application-specific, i.e., different applications may have different requirements on the level of robustness.% and depends on the required safety level. 

RobOT integrates the DL (re)training into the testing framework. 
It starts from the initial training dataset $D_0$, and trains an initial DNN $f_0$ in the standard way. 
Then, it applies a fuzzing algorithm (see Section~\ref{sec:test-gen}) which is guided by our proposed testing metrics (see Section~\ref{sec:metrics})
to generate a new set of test cases $D_{t}$, for retraining the model $f_0$ to improve its adversarial robustness. 
The retraining step distinguishes RobOT from existing DL testing works and it places a specific requirement on how the test cases in $D_{t}$ are generated and selected, i.e., the test cases must be helpful in improving $f_0$'s robustness after retraining. We discuss how the test cases are generated in the rest of this section.

RobOT iteratively generates the test suite $D_{t}$ and retrains the model $f_{n}$ at each iteration. Afterwards, it checks whether the robustness of the new model $f_n$ is satisfactory using an independent adversarial validation dataset $D_v$, subject to an acceptable degrade of the model's accuracy on normal/non-adversarial data. If the answer is yes, it terminates and outputs the final model $f_{n}$; otherwise, RobOT continues until the model robustness is satisfactory or a predefined testing budget is reached. In the following, we illustrate each component of RobOT in detail.   



% \begin{definition} \textbf{\textit{Utility}} Given a DL model $f:D\to C$ and a set of properties $E$ on the model, the model utility $U:(f,E)\to [0,1]$ is a function measuring the fitness of $f$ with respect to $E$.        
% \end{definition}

% The set of `properties' reflects different aspects of a DL model of concern such as accuracy, robustness, fairness, etc. We refer the readers to \cite{testing-survey} for detailed definitions for different properties. 

\subsection{DL Robustness: A Formal Definition}
\label{sec:robustness}
Although many DL testing works in the literature claim a \emph{potential} improvement on the DL model robustness by retraining using the test suite generated, such a conjecture is often not rigorously examined. This is partially due to the ambiguous definition of robustness. For instance, the evaluations of \cite{deepxplore,deeptest,concolic,deephunter} are based on accuracy, in particular empirical accuracy on the validation set~\cite{testing-survey}, rather than robustness. In RobOT, we focus on improving the model \emph{robustness} (without sacrificing accuracy significantly), and we begin with defining robustness.
% and remark that our testing framework can be easily adapted to other properties as well.
% \vspace{1mm}
\begin{definition} \textbf{\textit{Global Robustness (GR)}} Given an input region $R$, a DL model $f:R\to Y$ is $(\sigma,\epsilon)$-globally-robust iff $\forall x_1,x_2\in R, ||x_1-x_2||_p\le\sigma \Rightarrow\ ||f(x_1)-f(x_2)||\le\epsilon$. $\hfill \square$
\end{definition}

Global robustness is theoretically sound, and yet extremely challenging for testing or verification~\cite{katz2017towards}. 
To mitigate the complexity, multiple attempts have been made to constrain the robustness into local input space, such as Local Robustness~\cite{huang2017safety}, CLEVER~\cite{clever} and Lipschitz Constant~\cite{xu2012robustness}. These local versions of robustness are however not ideal either, i.e., they have been shown to have their own limitations~\cite{lc_lim,katz2017towards}. For instance, CLEVER relies on the extreme value theory, making it extremely costly to calculate. 

In RobOT, we adopt a practical empirical definition of robustness, which has been commonly used for model robustness evaluation in the machine learning literature
\cite{pgd,pgd-con,zhang2019theoretically,wang2019improving,carlini2019evaluating}.

% \vspace{1mm}
\begin{definition} \label{def:empirical-robustness}\textbf{\textit{Empirical Robustness (ER)}} Given a DL model $f:X\to Y$ and a validation dataset $D_v$, we define its empirical robustness $\mu:(f,D_v,ATT)\to [0,1]$ as $\gamma$, where $ATT$ denotes a given type of adversarial attack and $\gamma$ is the accuracy of $f$ on the adversarial examples obtained by conducting $ATT$ on $\langle D_v,f\rangle$. $\hfill \square$
\end{definition}

% Notice that \emph{empirical robustness} can be viewed as the model utility with respect to the robustness property. 
Intuitively, Def. \ref{def:empirical-robustness} evaluates a model's robustness using its accuracy on the adversarial examples crafted from a validation set $D_v$. Such an empirical view of DL robustness is testing-friendly and it facilitates RobOT to efficiently compare the robustness of the models before and after testing and retraining.  Definition~\ref{def:empirical-robustness} is also practical, as it connects the DL robustness with many existing adversarial attacks (such as~\cite{fgsm,pgd,cw}) as a part of the definition.
% A model may have different resilience to different attacks. 
In particular, for the evaluation of RobOT in Section \ref{sec:exp}, we use two popular attacks, i.e., FGSM \cite{fgsm} and PGD (Projected Gradient Descent) \cite{pgd} as $ATT$.   

%For a fair robustness comparison,
 % (for a same task), 
%we favor configurable adversarial attacks so that we can set the same attack parameter, e.g., step size or amount of perturbation. In practice, we use two popular attacks, i.e., FGSM \cite{fgsm} and PGD (Projected Gradient Descent) \cite{pgd} as $ATT$.  

\subsection{RobOT DL Testing: A General View}

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{testing}
\caption{Comparison between traditional and deep learning system quality assurance by testing.}
\label{fig:compar}
\end{figure}

We first compare and highlight the difference between testing traditional software and deep learning systems in Fig.~\ref{fig:compar}. While many testing methods (like random testing~\cite{randoop}, symbolic execution~\cite{klee}, concolic testing~\cite{wang2018towards} and fuzzing \cite{fuzz}) can be applied to identify vulnerabilities or bugs for both the traditional software and the DL systems, the workflow differs for the two after testing is done, i.e.,
%For traditional software, commonly used testing methods include random testing \cite{randoop}, symbolic execution \cite{klee}, concolic testing \cite{wang2018towards} and fuzzing \cite{fuzz}. Recently, many of these approaches have been adapted to the setting of testing deep learning models \cite{concolic,adapt,deephunter}. In the second phase, 
the quality of traditional software is enhanced by patching the found bugs, whereas deep learning systems are improved via retraining.  %with the test cases generated. 
Arguably, the ultimate goal of testing is to improve the system's quality. Such improvement is guaranteed by patching bugs identified through testing in traditional software (assuming regression bugs are not frequent), i.e., the usefulness of a bug-revealing test for traditional software requires no justification. It is not obvious for DL systems, i.e., the usefulness of a test case can only be judged by taking into account the retraining step. Nevertheless, the retraining phase is largely overlooked so far in the deep learning testing literature.

Based on the Empirical Robustness definition in Def.~\ref{def:empirical-robustness}, in Alg.~\ref{alg:main}, we present the high level algorithmic design of RobOT for the workflow of DL testing in Figure \ref{fig:compar}. The initial trained model $f_0$ is given as an input in the algorithm and the testing and retraining iterations in RobOT are conducted within the main loop (Lines 2-6). The loop continues until the user-provided empirical robustness requirement is satisfied (Line 2). 

RobOT aims to bridge the gap between the DL testing and retraining. Let $T$ (Line 3) denote a fuzzing algorithm to generate test cases (guided by certain metrics). The objective of robustness-oriented testing is to improve the model robustness by testing. Formally, given a deep learning model $f$, the goal of RobOT at each iteration is to improve the following:
\begin{equation}
ER(\argmin_\theta\frac{1}{n}\sum_{i=1}^n\mathcal{J}_{(x_i,y_i)\in D\cup T(f,D)}(\theta,x_i,y_i)).
\end{equation} 
Intuitively, the testing metric should be designed in such a way that after retraining with the generated test cases, the model robustness is improved. This objective directly links the testing metric to the model robustness.

%Inside the loop, FOL-Fuzz (Line 2) will be our proposed fuzzing test generation. 
In the remaining of this section, we realize the method in Line 3 by answering the question: \emph{how should we design test metrics that are strongly correlated with the model robustness and how can we generate test cases guided by the proposed metrics?}

% \todo{The writing can be improved with a running example to explain each concept and step in Section III.}

% While most existing test case generation algorithms are guided by coverage metrics \cite{deepxplore,deephunter,adapt}, multiple recent studies have shown 
%This is motivated by the limited correlation between existing neuron coverage metrics and the model robustness \cite{misleading,limit}, which throws shadow on the usefulness of the test cases generated in this way in improving the model robustness. 

\begin{algorithm}[t]
\caption{RobOT($f_0,D,D_v,r,t$)}
\label{alg:main}
\begin{algorithmic}[1]
	\State $f=f_0$
	\While{$ER(f,D_v,t)<r$} % and not exceed testing budget}
		\State $D_t \leftarrow T(f, D)$ %Apply metric-guided fuzzing on $(f,D)$ to generate a set of test cases $D_t$
		\State $D \leftarrow D \cup D_t$
		\State Update $f$ by retraining the model with $D$
	\EndWhile
	% \State Output $f$\;
	% \State Let $\mathbb{I}$ be the input domain
	% \For{$x_{i} \in x$}
	% 	\State $x_{i} = \max(x_{i}, \mathbb{I}_{i}.min)$
	% 	\State $x_{i} = \min(x_{i}, \mathbb{I}_{i}.max)$
	% 	\If{$sign(grad_{a}) = sign(grad'_{a})$}
	% 	    		\State $dir_{a} = sign(grad_{a})$
	% 	\EndIf
	% \EndFor
	\State \Return $f$
\end{algorithmic}
\end{algorithm}

% \begin{definition} \textbf{\textit{Model-improvement Mechanism (MIM)}} Given a machine learning model $f:D\to C$ and a set of adversarial samples $D_{adv}$ of $f$, a model improvement mechanism is a function $M:(f,D_{adv})\to f$, which outputs an improved model $f'$ (in terms of a certain utility $u\in U$) with the combined dataset $D\cup D_{adv}$.   
% \end{definition}

% We focus on two most commonly adopted MIMs, i.e., retraining \cite{deepxplore,deephunter,concolic,deeptest} and adversarial training \cite{adv-train,pgd}. In the framework shown in Figure~\ref{fig:frame}, we assume that after obtaining the testing data, one MIM is chosen to update the model. 

% \begin{definition} \textbf{\textit{Convergence}} A testing procedure is $(\epsilon,e,m)-converged$ iff $||U(m(f,D_{adv}),e)-U(f,e)||\le\epsilon$, where $e\in E$ is a given property and $m\in M$ is a model-improvement mechanism.
%   % (training set, adversarial sample set, mechanism, utility)
% \end{definition}

% With ambiguity, we target robustness property analysis in the following and omit $e$.

% \commentout{
% \subsection{Revisit Deep Learning Testing: A Unified View} First, we aim to provide a unified view of testing in the quality assurance of deep learning software for better designing the metrics. Fig.~\ref{fig:compar} shows a comparison between testing traditional software and deep learning systems. They both consist of two phases. In the first phase, a testing method is applied to identify vulnerabilities/bugs of the system. For traditional software, commonly used testing methods include random testing \cite{randoop}, symbolic execution \cite{klee}, concolic testing \cite{wang2018towards} and fuzzing \cite{fuzz}. Recently, many of these approaches have been adapted to the setting of testing deep learning models \cite{concolic,adapt,deephunter}. In the second phase, the quality of traditional software is enhanced by patching the found bugs while deep learning models are often improved by retraining with the test cases generated. The second phase, i.e., improving the original deep learning software, is largely overlooked so far in the deep learning testing literature.

% RobOT aims to bridge the gap by considering the second phase in testing DL systems. Let $T$ denote a fuzzing algorithm to generate test cases guided by $T_m$ (the testing metric for $T$). The objective of robustness-oriented testing is to improve the model robustness by testing. Formally, given a deep learning model $f$, the goal of RobOT at each iteration is to improve:
% \begin{equation}
% ER(\argmin_\theta\frac{1}{n}\sum_{i=1}^n\mathcal{J}_{(x_i,y_i)\in D\cup T(f,D)}(\theta,x_i,y_i))
% \end{equation} 
% Intuitively, the testing metric should be designed such that after retraining with the generated test cases guided by the testing metric, the model robustness should be improved. This objective asks for directly linking the testing metric with the model robustness.
% % , which is often either missing \cite{} or proved to be ineffective \cite{}. 
% }


\subsection{Robustness-Oriented Testing Metrics} 
\label{sec:metrics}
Our goal is to design testing metrics which are strongly correlated with model robustness. We note that there have been some efforts in the machine learning community to modify the standard training procedure in order to obtain a more robust model. For instance, the most effective and successful approach so far is robust training, which incorporates an adversary in the training process so that the trained model can be robust by minimizing the loss of adversarial examples in the first place \cite{pgd}:
\begin{equation}
\min_\theta\frac{1}{n}\sum_{i=1}^n\max_{||x'_i-x_i||_p\le\epsilon}\mathcal{J}(f(\theta,x'_i),y_i).
\end{equation}

At the heart of robust training is to identify a \emph{strong} (ideally worst-case) adversarial example $x'$ around\footnote{A $\epsilon-$ball defined according to a certain $L_p$ norm.} a normal example $x$ and train the model so that the loss on the strong adversarial example can be minimized. Robust training has shown encouraging results in training more robust models~\cite{pgd,pgd-con}. This inspires us to consider deep learning testing analogously in terms of how we generate test cases (around a normal example) and retrain the model with the test cases to improve the model robustness. The key implication is that when we design robustness-oriented testing metrics to guide testing, we should evaluate the usefulness of a test case from a loss-oriented perspective. 
% which is immediately relevant to improving the model robustness through retraining.

% \subsubsection{Metrics} 
% Specifically, we aim to design a set of testing metrics which would achieve the following goals. First, the metric should be well correlated with the model robustness. Second, the metric should be able to quantify how good a test case is in improving the model robustness through retraining. In a nutshell, the metric will guide us to identify the most valuable test cases in improving the model robustness. In the following, we introduce such a metric. 

Let $x_0$ be the seed for testing. We assume that a test case $x^t$ is generated in the neighborhood $\epsilon-$ball around $x_0$, i.e., $\{x|\ ||x-x_0||_p\le\epsilon\}$ using either a testing method or an adversarial attack. The main intuition is that a test case which induces a higher loss is a stronger adversarial example, which is consequently more helpful in training robust models~\cite{pgd}. Based on this intuition, we propose two levels of testing metrics on top of the loss as follows.
% \jy{this intuition needs to be expanded} 

\paragraph{Zero-Order Loss (ZOL)} The first metric directly calculates the loss of a test case with respect to the DL model. Formally, given a test case $x^t$ (generated from seed $x$), a DL model $f$, the loss of $x^t$ on $f$ is defined as:
\begin{equation}
ZOL(x^t,f)=\mathcal{J}(f(\theta,x^t),y),
\end{equation}
where $y$ is the ground-truth label of $x$. For test cases generated from the same seed, we prefer test cases with higher loss, which are more helpful in improving the model robustness via retraining.

\paragraph{First-Order Loss (FOL)} The loss of generated test cases can be quite different for different seeds. In general, it is easier to generate test cases with high loss around seeds which unfortunately do not generalize well. Thus, ZOL is unable to measure the value of the test cases in a unified way. To address this problem, we propose a more fine-grained metric which could help us measure to what degree we have achieved the highest loss in the seed's neighborhood. The intuition is that, given a seed input, the loss around it often first increases and eventually converges if we follow the gradient direction to modify the seed~\cite{pgd}. Thus, a criteria which measures how well the loss converges can serve as the testing metric. A test case with better convergence quality corresponds to a higher loss than its neighbors. Next, we introduce First-Order Stationary Condition (FOSC) to provide a measurement on the loss convergence quality of the generated test cases. 
% We will show that FOSC is strongly-correlated with adversarial strength of the test cases. Meanwhile, FOSC is also a good indicator of the model robustness after retraining. 
% In the following, we present FOSC in details. 

Formally, given a seed input $x_0$, its neighborhood area $\mathcal{X}=\{x|\ ||x-x_0||_p\le\epsilon\}$, and a test case $x^t$, the FOSC value of $x^t$ is calculated as:
\begin{equation}
\label{eq:fosc}
c(x^t)= \text{max}_{x\in \mathcal{X}}\langle x-x^t,\nabla_x f(\theta,x^t)\rangle.
\end{equation}

In~\cite{pgd-con}, it is proved that the above problem has the following closed form solution if we take the $\infty-$norm for $\mathcal{X}$.
\begin{equation}
\label{eq:fosc:sol1}
c(x^t)=\epsilon||\nabla_x f(\theta,x^t)||_1-\langle x^t-x_0,\nabla_x f(\theta,x^t)\rangle.
\end{equation}

However, many existing DL testing works are generating test cases from the $L_2$ norm neighborhood which makes the above closed-form solution for $L_\infty$ infeasible. We thus consider solving the formulation in Eq. \ref{eq:fosc} with $L_2$ norm and obtain the solution as follows:
\begin{equation}
\label{eq:fosc:sol2}
c(x^t)=\epsilon||\nabla_x f(\theta,x^t)||_2.
\end{equation}

\begin{proof}
According to Cauchy–Schwarz inequality:

\begin{align*}
|\langle x-x^t,\nabla_x f(\theta,x^t)\rangle|^2\le\\ 
\langle x-x^t,x-x^t\rangle \cdot \langle \nabla_x f(\theta,x^t),\nabla_x f(\theta,x^t)\rangle\le\\
\epsilon^2\cdot (||\nabla_x f(\theta,x^t)||_2)^2
\end{align*}

Since there must exist $x^t$ such that $x-x^t$ and $\nabla_x f(\theta,x^t)$ are in the same direction, we thus have:
\begin{align*}
\max|\langle x-x^t,\nabla_x f(\theta,x^t)\rangle|^2=\epsilon^2\cdot(||\nabla_x f(\theta,x^t)||_2)^2
\end{align*}
Thus,
\begin{align*}
\max|\langle x-x^t,\nabla_x f(\theta,x^t)\rangle|=\epsilon\cdot ||\nabla_x f(\theta,x^t)||_2
\end{align*}
\end{proof}


Note that FOSC (in both Eq.~\ref{eq:fosc:sol1} and Eq. \ref{eq:fosc:sol2}) is cheap to calculate, whose main cost is a one-time gradient computation (easy to obtain by all the DL frameworks). The FOSC value represents the first-order loss of a given test case. The loss of a test case converges and achieves the highest value if its FOSC value equals zero. Thus, a smaller FOSC value means a better convergence quality and a higher loss. 

% , where $\epsilon$ is the imposed perturbation to generate $x^t$ from $x_0$
% Note that FOSC is cheap to calculate using Eq.~\ref{eq:fosc} whose main cost is a one-time gradient computation by back-propagation. The FOSC value represents the first-order loss of a given test case. The loss of a test case converges and achieves the highest if its FOSC value equals zero. Thus, a smaller FOSC value means a better convergence quality and a higher loss. 
% and a higher loss, and thus preferred for retraining. 
% Specifically, the FOSC value of a test case achieves zero (which stands for optimal convergence quality) under two conditions:
% \begin{itemize}
% 	\item \textbf{Case 1)} $\nabla_x f(\theta,x^t)=0$, which means the test case is a stationary point which has maximum loss in $\mathcal{X}$.
% 	\item \textbf{Case 2)} $x^t-x_0=\epsilon\cdot \text{sign}(\nabla_x f(\theta,x^t))$, which means the local minimum point of $f(\theta,x^t)$ is reached on the boundary of $\mathcal{X}$.
% \end{itemize} 

% Fig.~\ref{fig:fosc} shows the two cases from our experiment. 

% However, most existing testing works use $L_2$ norm to define the neighborhood.  


% However, its performance highly relies on the quality of the found adversarial example \cite{}.

\paragraph{Comparison with Neuron Coverage Metrics} 
Compared to neuron coverage metrics, our proposed loss based metrics have the following main differences. First, both ZOL and FOL are strongly correlated to the adversarial strength
% \todo{not sure what you mean by "adversarial strength". Remove it otherwise} 
of the generated test cases and the model robustness. Thus, our metrics can serve as strong indicators on the model's robustness after retraining. Meanwhile, our metrics are also able to measure the value of each test case in retraining, which helps us select valuable test cases from a large amount of test cases to reduce the retraining cost.

% 3) easy to calculate or profile

\subsection{FOL Guided Test Case Selection} In the following, we show the usefulness of the proposed metric through an important application, i.e., test case selection from a massive amount of test cases. Note that by default, we use the FOL metric hereafter due to the limitation of ZOL as described above. Test case selection is crucial for improving the model robustness with limited retraining budget. The key of test case selection is to quantitatively measure the value of each test case. So far this problem remains an open challenge. Prior work like DeepGini has proposed to calculate a Gini index of a test case from the model's output probability distribution~\cite{deepgini}. DeepGini's intuition is to favor those test cases with most uncertainty (e.g., a more flat distribution) under the current model's prediction. Compared to DeepGini, FOL contains fine-grained information at the loss level and is strongly correlated with model robustness. 

Given a set of test cases $D^t$, we introduce two strategies based on FOL to select a smaller set $D^s\subset D^t$ for retraining the model as follows. Let $D^t=[x_1,x_2,\cdots,x_m]$ be a ranked list in descending order by FOL value, i.e., $FOL(x_i)\ge FOL(x_{i+1})$ for $i\in[1,m-1]$.

\begin{algorithm}[t]
\caption{KM-ST($D^t,k,n$)}
\label{alg:kmst}

\begin{algorithmic}[1]
\State $D^s=\emptyset$
\State Let $max$ and $min$ be the maximum and minimum FOL value respectively
\State Equally divide range $[min,max]$ into $k$ sections $KR=[R_1,R_2,\cdots,R_k]$
% \State Categorize $D^t$ into $k$ sections according to 
% \State Divide $D^t$ into $k$ consecutive sections
\For{Each FOL range $r\in[R_1,R_2,\cdots,R_k]$}
	\State Randomly select $n/k$ samples $D^r$ from $D^t$ whose FOL values are in $r$
	\State $D^s=D^s\cup D^r$
% 	\State $seed\_list=[x]$
% 	\While{$len(seed\_list)>0$}
% 		\State $xs=seed\_list.pop()$
% 	\EndWhile
\EndFor
	\State \Return $D^s$
\end{algorithmic}
\end{algorithm}


% \begin{itemize}
	% \item Random Strategy (Ra-ST). This is the baseline strategy where we randomly select $D^s$ from $D^t$.
	% \item 
\paragraph{K-Multisection Strategy (KM-ST)} The idea of KM-ST is to uniformly sample the FOL space of $D^t$. Algo. \ref{alg:kmst} shows the details. Assume we need to select $n$ test cases from $D^t$. We equally divide the range of FOL into $k$ sections ($KR$) at line 3. 
% and categorize $D^t$ into $k$ consecutive sections. 
Then for each range $r\in KR$, we randomly select the same number of test cases at line 5.  




\paragraph{Bi-End Strategy (BE-ST)} The idea of BE-ST is to form $D^s$ by equally combining test cases with small and large FOSC values. This strategy mixes test cases of strong and weak adversarial strength, which is inspired by a recent work on improving standard robust training~\cite{khoury2019adversarial}. Given a ranked $D^t$, we can simply take an equal number of test cases from the two ends of the list to compose $D^s$.  


\begin{figure*}[t]
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=	1.45in]{figs/mnist_loss_st.pdf}
   % \caption{NASA Logo} 
   \label{fig:st:mnist}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/fashion_loss_st.pdf}
   % \caption{Orion Logo} 
   \label{fig:st:fashion}
\end{subfigure}%
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/svhn_loss_st.pdf}
   % \caption{NASA Logo} 
   \label{fig:st:svhn}
\end{subfigure}% 
\begin{subfigure}[b]{0.25\textwidth}
   \centering 
   \includegraphics[height=1.45in]{figs/cifar_loss_st.pdf}
   % \caption{Orion Logo} 
   \label{fig:st:cifar}
\end{subfigure}%
   \caption{Loss of selected test cases for different datasets using different strategies.}
   \label{fig:loss:st}
\end{figure*}

Figure~\ref{fig:loss:st} shows the loss map of the selected test cases according to different strategies. We could observe that BE-ST prefers test cases of higher loss, KM-ST uniformly samples the loss space, while DeepGini often prefers test cases with lower loss.
 % relationship between our strategy and the loss of the test cases.
% \jy{missing figure and explanation}
% adaption to testing $L_2$ norm



\subsection{FOL Guided Fuzzing} 
\label{sec:test-gen}

Next, we introduce a simple yet efficient fuzzing strategy to generate test cases based on FOL. Note that since we have no prior knowledge of the FOL distribution, we are not able to design fuzzing strategy for KM-ST. Instead, we design a fuzzing algorithm for the BE-ST strategy. The idea is to greedily search for test cases in two directions, i.e., with both small or large FOL values.
% \todo{DX: both?} 

Algo.~\ref{alg:fuzz} presents the details. The inputs include the model $f$, the list of seeds to fuzz $seeds\_list$, the fuzzing region $\epsilon$, the threshold on the small FOL value $\xi$, the number of labels to optimize $k$, a hyper-parameter $\lambda$ on how much we favor FOL during fuzzing and lastly the maximum number of iterations to fuzz for a seed $iters$. For each seed in the list, we maintain a list of seeds $s\_list$ at line 3. After obtaining a seed $x$ from $s\_list$ (line 5), we iteratively add perturbation on it from line 8 to line 28 in a way guided by FOL. We set the following objective for optimization (line 9).
% \todo{DX:obj to Obj}
\begin{equation}
\label{eq:obj}
obj=\sum_{i=2}^k P(c_i)-P(c_1)+\lambda \cdot FOL(x')
\end{equation}   
, where $c_i$ is the label with the $i^{\text{th}}$ largest softmax probability of $f$ ($c_1$ with the maximum), $P(c)$ is the softmax output of label $c$ and $k$ is a hyper-parameter. The idea is to guide perturbation towards changing the original label (i.e., generating an adversarial example) whilst increasing the FOL value. We then obtain the gradient of the objective (line 10) and calculate the perturbation based on the gradient by multiplying a learning rate and a randomized coefficient (0.5 to 1.5) to avoid duplicate perturbation (line 11). We run two kinds of checks to achieve the BE-ST strategy at line 15 and line 22 respectively. If the FOL value of the new sample after perturbation (x') is either increasing (line 15) or is smaller than a threshold (line 22), we add $x'$ to the seed list (line 17 and line 23). Furthermore, we add $x'$ to the fuzzing result if it satisfies the check and has a different label with the original seed $x$ (line 19 and line 25). Note that compared to neuron coverage guided fuzzing algorithms which need to profile and update neuron coverage information~\cite{adapt,deephunter}, our FOL guided fuzzing algorithm is much more lightweight, i.e., whose main cost is to calculate a gradient at each step. 

\begin{algorithm}[t]
\caption{FOL-Fuzz($f,seeds\_list,\epsilon,\xi,k,\lambda,iters$)}
\label{alg:fuzz}

\begin{algorithmic}[1]
% \State Let $seeds\_list$ be a list of seeds to fuzz
\State Let $fuzz\_result=\emptyset$
\For{$seed\in seeds\_list$}
	\State Maintain a list $s\_list=[seed]$
	\While{$s\_list$ is not empty}
		\State Obtain a seed $x=s\_list.pop()$
		\State Obtain the label of the seed $c_1=f(x)$
		% \State $c, c_{topk} = dnn.predict(xs)$
		% \State Calculate $FOL(x)$ 
		% \State Let $FOL_c=FOL(x)$
		\State Let $x'=x$
		\For{$iter=0$ to $iters$}
			\State Set optimization objective $obj$ using Eq.~\ref{eq:obj}
			\State Obtain $grads = \frac{\nabla obj}{\nabla x'}$
			\State Obtain $perb = processing(grads)$
			\State Let $x’ = x' + perb$
			\State Let $c'= f(x’)$
			\State Let $dis = Dist(x’, x)$
			\If{$FOL(x')\ge FOL_m$ and $dis\le\epsilon$}
				\State $FOL_m=FOL(x')$
				\State $s\_list.append(x')$
				\If{$c'!=c_1$}
				\State $fuzz\_result.append(x')$
				\EndIf
			\EndIf
			\If{$FOL(x')<\xi$ and $dis\le\epsilon$}
				\State $s\_list.append(x')$
				\If{$c'!=c_1$}
				\State $fuzz\_result.append(x')$
				\EndIf
			\EndIf
		\EndFor

	\EndWhile
\EndFor
	% \While{$U(f,D_v)<r$ and not exceed testing budget}
	% 	\State Apply $t$ on $f,D$ to generate a set of test cases $D_t$
	% 	\State $D=D\cup D_t$
	% 	\State Update $f$ by retraining the model with $D$
	% \EndWhile
	% % \State Output $f$\;
	% % \State Let $\mathbb{I}$ be the input domain
	% % \For{$x_{i} \in x$}
	% % 	\State $x_{i} = \max(x_{i}, \mathbb{I}_{i}.min)$
	% % 	\State $x_{i} = \min(x_{i}, \mathbb{I}_{i}.max)$
	% % 	\If{$sign(grad_{a}) = sign(grad'_{a})$}
	% % 	    		\State $dir_{a} = sign(grad_{a})$
	% % 	\EndIf
	% % \EndFor
\State \Return $fuzz\_result$
\end{algorithmic}
\end{algorithm}

==> icse21 2/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \cite{year no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> icse21 2/Related_Work.tex <==
\section{Related works}
\label{sec:rel}

This work is mainly related to the following lines of works on building more robust deep learning systems.

\paragraph{Deep Learning Testing} Extensive DL testing works are focused on designing testing metrics to expose the vulnerabilities of DL systems including neuron coverage \cite{deepxplore}, multi-granularity neuron coverage \cite{deepgauge}, neuron activation conditions \cite{concolic} and surprise adequacy~\cite{surprise}. Along with the testing metrics, many test case generation algorithms are also proposed including gradient-guided perturbation~\cite{deepxplore,adf}, black-box~\cite{feature_guided_test} and metric-guided fuzzing~\cite{deephunter,adapt,dlfuzz}. However, these testing works lack rigorous evaluation on their usefulness in improving the model robustness (although most of them claim so) and have been shown to be ineffective in multiple recent works \cite{limit,misleading,meaningless}. Multiple metrics have been proposed in the machine learning community to quantify the robustness of DL models as well \cite{xu2012robustness,weng2018towards,brendel2019accurate,clever}. However, most of them are used to evaluate local robustness and hard to calculate. Thus these metrics are not suitable to test directly. Our work bridges the gap by proposing the FOL metric which is strongly correlated with model robustness and integrate retraining into the testing pipeline for better quality assurance.
% However, testing can not provide any safety guarantee in general. There are also attempts to formally verify certain safety properties against the DNN to provide certain safety guarantees~\cite{safety_verify,reluplex,prove_robust,weng2018towards}.


% \paragraph{Robustness} 
% Besides, in~\cite{deepxplore} and the following work~\cite{dnn_test,ma2018deepgauge}, neuron coverage and its extensions are argued to be the key indicators of the DNN robustness. 
% In~\cite{measure_cons}, Bastani \textit{et al.} proposed adversarial frequency and adversarial severity as the robustness metrics and encode robustness as a linear program.  

\paragraph{Adversarial Training} 
The key idea of adversarial training is to improve the robustness of the DL models by considering adversarial examples in the training phase. There are plenty of works on conducting adversarial attacks on DL models (of which we are not able to cover all) to generate adversarial examples such as FGSM ~\cite{fgsm}, PGD \cite{pgd} and C\&W~\cite{cw}.  
% JSMA~\cite{jsma}, black-box attacks~\cite{bb} and others~\cite{su2018attacking,sharif2016accessorize,galloway2017attacking,brendel2017decision,xiao2018spatially}. 
% However, 
Adversarial training in general may overfit to the specific kinds of attacks which generate the adversarial examples for training~\cite{pgd} and thus can not guarantee robustness on new kinds of attacks. Later, robust training \cite{pgd} is proposed to train robust models by solving a saddle point problem described in Sec. \ref{sec:meth}. DL testing complements these works by generating more diverse adversarial examples. 

% \paragraph{Adversarial Sample Detection} Another direction is to automatically detect those adversarial samples that a DNN will mis-classify. One way is to train a `detector' subnetwork from normal samples and adversarial samples~\cite{detection_subnn}. Alternative detection algorithms are often based on the difference between how an adversarial sample and a normal sample would behave in the softmax output~\cite{feature_squezze,detection1,detection2,feinman2017detecting} or under random perturbations~\cite{detection_ours}. 




